Uni-Perceiver-MoE: Learning Sparse Generalist Models with Conditional MoEs

To build an artificial neural network like the biological intelligence system, recent works have unified numerous tasks into a generalist model, which can process various tasks with shared parameters and do not have any task-specific modules. While generalist models achieve promising results on various benchmarks, they have performance degradation on some tasks compared with task-specialized models. In this work, we find that interference among different tasks and modalities is the main factor to this phenomenon. To mitigate such interference, we introduce the Conditional Mixture-of-Experts (Conditional MoEs) to generalist models. Routing strategies under different levels of conditions are proposed to take both the training/inference cost and generalization ability into account. By incorporating the proposed Conditional MoEs, the recently proposed generalist model Uni-Perceiver can effectively mitigate the interference across tasks and modalities, and achieves state-of-the-art results on a series of downstream tasks via prompt tuning on 1% of downstream data. Moreover, the introduction of Conditional MoEs still holds the generalization ability of generalist models to conduct zero-shot inference on new tasks, e.g., video-text retrieval and video caption. Code and pre-trained generalist models shall be released.

==> tables/model_interference.tex <==
\begin{table}[t]
\small
    \centering
% \resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|ccccccc}

\toprule
Model & Layers & $\#$param & $\#$FLOPs &  training & IN1k & bookswiki & caption\\


\midrule

BERT\textsubscript{Medium} & 8  & 41M & 0 & single task\\
BERT\textsubscript{Medium} & 8 & 41M & 0 & multi-task\\
BERT\textsubscript{Base}  & 12 & 110M & 0 & single task\\
BERT\textsubscript{Base}  & 12  & 110M & 0 & multi-task\\
BERT\textsubscript{Large} & 24 & 340M & 0 & single task\\
BERT\textsubscript{Large} & 24  & 340M & 0 & multi-task\\
\bottomrule
\end{tabular}}
    % \caption{The datasets used in the pretrain stage are listed above. }
    \caption{The performance of  models with different model capacity under single task training or multitask training. We specify the number of transformer layers, the total number of parameters, the computation costs, the ImageNet-1K precision\@1(\%), the Perplexity on held-out bookswiki  data (ppl), and BLEU-4 on COCO caption.
    } 
    \label{tab:model_interference}
    \vspace{-1.2em}
\end{table}

==> tables/msrvtt.tex <==

\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{table}[t]
\centering
\small
    \caption{Video-text retrieval (novel task) Recall@1  on MSRVTT.}
    \label{tab:msvtt}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|rr|cccccc}
    \toprule
 \multirow{2}{*}{Method} &  & &   \multicolumn{3}{c}{Video $\rightarrow$ Text} &   \multicolumn{3}{c}{Text $\rightarrow$ Video}   \\
  & \#param & \#data  &  WT & PT\textsubscript{1\%}  & FT\textsubscript{100\%} & WT & PT\textsubscript{1\%}& FT\textsubscript{100\%}  \\
   \midrule
   CLIP4Clip~\citeappendix{luo2021clip4clip} & 210M & 400.4M & - &- & 42.7  &-  &- & 44.5 \\
  CLIP2video~\cite{fang2021clip2video}& 132M & 400M &- &- & 43.5  &-  &- & 45.6\\
  HunYuan\_tvr~\cite{min2022hunyuan_tvr}& 364M & 400M &- & -& 47.4& - &- & 49.7   \\
%   ORG-TRL\textsuperscript~\cite{zhang2020object} & 86M &2.0M &-& -&- &- &- \\
  \midrule
  %Uni-Perceiver-B~\cite{zhu2021uniperceiver} & 124M & 44.1M & 42.7 & 61.2 & 61.5 & 34.6 & 42.6 & 45.4 & 20.3 & 54.8 & 61.5  \\
 Uni-Perceiver-B & 124M & 44.1M&  \\
 + Conditional MoEs & 124M & 44.1M &  \\
 Uni-Perceiver-L & 354M & 44.1M&   \\
 + Conditional MoEs & 354M & 44.1M& 22.5 & 40.8 &45.7 & 23.6 & 39.7 & 44.4\\
   \bottomrule   
    \end{tabular}}
\vspace{-1.4em}
\end{table}



==> tables/multitask_with_MoE.tex <==
\begin{table}[t]
\small
    \centering
% \resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|cccccccc}

\toprule
Expert Number &  $\#$param & $\#$FLOPs &  experts & training-days & IN1k & bookswiki & caption\\


\midrule

1 & \\
2 &\\
4 &\\
8 & \\
16 & \\
\bottomrule
\end{tabular}}
    % \caption{The datasets used in the pretrain stage are listed above. }
    \caption{The expert number in MoE models.
    } 
    \label{tab:differentmoe}
    \vspace{-1.2em}
\end{table}

==> tables/survey.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.7}




\begin{table}[t]
\centering
\caption{
Training Cost of Related Works.  Related works are categorized into three classes: specialized models, integrated specialized models, and generalist models. We also list the specific types of training data used for training these methods from scratch, including the data to pre-train  the modality-specific encoders or the detectors for extracting region features. Note that the training data size does not include plain texts.
% In addition, the number of images is recorded as data size for detection datasets with instance annotations. 
}
\label{tab:comparison2}

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l| cccccc|c}
\toprule
\multirow{2}{*}{methods}             & \multicolumn{6}{c|}{traning data type} & \multirow{2}{*}{ training data size} \\
 & images &videos & image-text pairs & plain texts& bounding boxes & others & \\ 
                                                                       \midrule 
                      \midrule
 \multicolumn{7}{l}{$\blacktriangleright$ \textit{Specialized Models}} \\ \midrule
 ResNet~\cite{he2016deep} & \cmark &&&&& & 1.28M \\ \midrule
 DeiT~\cite{touvron2021training} &\cmark &&&& && 1.28M \\ \midrule
 ViT~\cite{steiner2021train} & \cmark &&&&& & 15.5M  \\  \midrule
 BERT~\cite{devlin2018bert}  &  & & & \cmark && & - \\ \midrule
  RoBERTa~\cite{liu2019roberta}  &  & & & \cmark & & & - \\ \midrule
  GPT~\cite{liu2021gpt} &  & & & \cmark &&  & - \\ \midrule
  Faster R-CNN~\cite{ren2015faster} & \cmark   & & &  &\cmark & & 1.4M \\ \midrule
  DETR~\citeappendix{carion2020end} & \cmark   & & &  &\cmark &   & 1.4M \\ \midrule
  Mask2Former~\cite{cheng2021mask2former} & \cmark   & & &  & & segmentation masks & 1.48M \\ \midrule
 TimeSformer~\cite{bertasius2021space} &\cmark &\cmark&&& &  &  14.5M \\ \midrule
VATT~\cite{akbari2021vatt} & &  & & & & audios; video-audio-text triplets & 138M \\ \midrule
ViViT~\cite{arnab2021vivit} &\cmark &\cmark&&& &  & 300.3M \\ \midrule
 CLIP~\cite{clip} &  & &\cmark&&  & & 400M \\ \midrule
 ALIGN~\cite{align} &  & &\cmark&&  & & 1.8B \\ \midrule
 ImageBERT~\cite{Qi2020ImageBERTCP} & & &\cmark&\cmark&  \cmark & & 13.8M \\ \midrule
 UNITER~\cite{chen2020uniter} &  & &\cmark&&   \cmark & instance attributes & 9.7M \\ \midrule
 ViLT~\cite{kim2021vilt} & \cmark & &\cmark&& &  & 25.2M \\ \midrule
 OSCAR~\cite{li2020oscar} &  & &\cmark&&  \cmark & instance attributes & 6.6M  \\ \midrule
 Unified VLP~\cite{zhou2020unified} &  & &\cmark&\cmark&   \cmark &  & 3.1M \\ \midrule
 HunYuan\_tvr~\cite{min2022hunyuan_tvr} &   & &\cmark&&   && 400M \\ \midrule
 CLIP2video~\cite{fang2021clip2video} &   & &\cmark&&   && 400M \\ \midrule
 ORG-TRL~\cite{zhang2020object} &  \cmark & \cmark&&\cmark&   \cmark &  & 1.6M \\ \midrule
BLIP~\cite{li2022blip} &  \cmark & &\cmark&\cmark& & & 144M \\ \midrule
CLIP-VIL~\cite{shen2021much} &  & &\cmark&&  & & 400M \\ \midrule

 
 \midrule
 
  \multicolumn{7}{l}{$\blacktriangleright$ \textit{Integrated Specialized Models}} \\ \midrule
 Florence~\cite{yuan2021florence} &  & &\cmark&&  \cmark &  & 909M  \\  \midrule
  FLAVA~\cite{singh2021flava} & \cmark& &\cmark&\cmark& &   & 71.3M \\  \midrule
INTERN~\cite{shao2021intern} & \cmark & &\cmark&&  \cmark & segmentation masks  & 10B \\
\midrule




 \midrule
 
  \multicolumn{7}{l}{$\blacktriangleright$ \textit{Generalist Models}} \\ \midrule
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uni-Perceiver~\cite{zhu2021uniperceiver} \& \\  Uni-Perceiver-MoE\end{tabular}} &  \multirow{2}{*}{\cmark}  &  \multirow{2}{*}{\cmark} & \multirow{2}{*}{\cmark}&  \multirow{2}{*}{\cmark}& &  &  \multirow{2}{*}{44.1M } \\ 
  & & & & & &   \\ \midrule
  \multirow{2}{*}{OFA~\cite{wang2022unifying}} &  \multirow{2}{*}{\cmark}  &  & \multirow{2}{*}{\cmark}&  \multirow{2}{*}{\cmark}& \multirow{2}{*}{\cmark}& \multirow{2}{*}{\begin{tabular}[c|]{@{}l@{}}visual question answering; \\ image-instance-text triplets\end{tabular}} &  \multirow{2}{*}{60.6M} \\
  &  &  &  &  &  &  \\ \midrule
  
     UNICORN~\cite{unicorn} & \cmark & &\cmark&\cmark&  & &  25.3M \\ \midrule
  
%  \multirow{2}{*}{OFA~\cite{wang2022unifying}} & \multirow{2}{*}{\begin{tabular}[c|]{@{}l@{}}visual question answering;  bounding boxes; \\ image-instance-text triplets;\end{tabular}} & \multirow{2}{*}{60.6M} \\ 
%  & & \\ \midrule
 CoCa~\cite{yu2022coca} & & &\cmark&&   & &  4.8B \\ \midrule
 Flamingo~\cite{alayrac2022flamingo} &  & &\cmark&& &  video-text pairs & 2.3B \\ \midrule
  SimVLM~\cite{wang2021simvlm} & & &\cmark&\cmark& &  & 1.8B \\ \midrule
   Gato~\cite{Gato} &  & &\cmark&& &  simulated data for control tasks& 2.16B \\ 
   
   
 
 
 
       
                      
                      \bottomrule
\end{tabular}
}

\end{table}

==> tables/survey_bak.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.7}




\begin{table}[t]
\centering
\caption{
Taxonomy of Related Works.
% In addition, the number of images is recorded as data size for detection datasets with instance annotations. 
}
\label{tab:comparison2}

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l| c|c}
\toprule
methods               & traning data type &training data size 
                                                                      \\ \midrule 
                      \midrule
 \multicolumn{3}{c}{Specialized Models} \\ \midrule
 ResNet~\citeappendix{he2016deep} & images & 1.28M \\ \midrule
 DeiT~\cite{touvron2021training} & images & 1.28M \\ \midrule
 ViT~\cite{steiner2021train} & images & 15.5M  \\  \midrule
 BERT~\cite{devlin2018bert}  & plain texts & - \\ \midrule
  RoBERTa~\cite{liu2019roberta}  & plain texts & - \\ \midrule
  GPT~\cite{liu2021gpt} & plain texts & - \\ \midrule
  Faster R-CNN~\cite{ren2015faster} & images; bounding boxes & 1.4M \\ \midrule
  DETR~\citeappendix{carion2020end} & images; bounding boxes & 1.4M \\ \midrule
  Mask2Former~\citeappendix{cheng2021mask2former} & images; segmentation masks & 1.48M \\ \midrule
 TimeSformer~\cite{bertasius2021space} &images; videos &  14.5M \\ \midrule
VATT~\cite{akbari2021vatt} & audios; video-audio-text triplets & 138M \\ \midrule
ViViT~\cite{arnab2021vivit} & images; videos & 300.3M \\ \midrule
 CLIP~\cite{clip} & image-text  pairs & 400M \\ \midrule
 ALIGN~\cite{align} & image-text pairs & 1.8B \\ \midrule
 ImageBERT~\cite{Qi2020ImageBERTCP} & image-text pairs; bounding boxes; plain texts & 13.8K \\ \midrule
 UNITER~\cite{chen2020uniter} & image-text pairs; bounding boxes+attributes & 9.7M \\ \midrule
 ViLT~\cite{kim2021vilt} & image-text pairs; images & 25.2M \\ \midrule
 OSCAR~\cite{li2020oscar} & image-text pairs; bounding boxes+attributes & 6.6M  \\ \midrule
 Unified VLP~\cite{zhou2020unified} & image-text pairs; bounding boxes; plain texts & 3.1M \\ \midrule
 HunYuan\_tvr~\cite{min2022hunyuan_tvr} & image-text pairs & 400M \\ \midrule
 CLIP2video~\cite{fang2021clip2video} & image-text pairs & 400M \\ \midrule
 ORG-TRL~\cite{zhang2020object} & images; videos; bounding boxes; plain texts & 1.6M \\ \midrule
BLIP~\cite{li2022blip} &image-text pairs; images; plain texts & 144M \\ \midrule
CLIP-VIL~\cite{shen2021much} & image-text pairs & 400M \\ \midrule

 
 \midrule
 
  \multicolumn{3}{c}{Integrated Specialized Models} \\ \midrule
 Florence~\cite{yuan2021florence} & image-text pairs; bounding boxes & 909M  \\  \midrule
  FLAVA~\cite{singh2021flava} &image-text pairs; images; plain texts & 71.3M \\  \midrule
INTERN~\cite{shao2021intern} & image-text pairs; images; bounding boxes; segmentation masks  & 10B \\ \midrule



 \midrule
 
  \multicolumn{3}{c}{Generalist Models} \\ \midrule
 Uni-Perceiver~\cite{yuan2021florence} & image-text pairs; images; videos; plain texts & 44.1M  \\ \midrule
 \multirow{2}{*}{OFA~\cite{wang2022unifying}} & \multirow{2}{*}{\begin{tabular}[c|]{@{}l@{}}image-text pairs; visual question answering; images; \\ image-instance-text triplets; bounding boxes;  plain texts\end{tabular}} & \multirow{2}{*}{60.6M} \\ 
 & & \\ \midrule
 CoCa~\cite{yu2022coca} & image-text pair & 4.8B \\ \midrule
 Flamingo~\cite{alayrac2022flamingo} & image-text pairs; video-text pairs & 2.3B \\ \midrule
  SimVLM~\cite{wang2021simvlm} &image-text pair; plain texts & 1.8B \\ \midrule
   UNICORN~\cite{unicorn} & image-text pairs; images; plain texts; &  25.3M \\ \midrule
   Gato~\cite{Gato} & simulated data for control tasks; image-text pairs & 2.16B \\ 
   
   
 
 
 
       
                      
                      \bottomrule
\end{tabular}
}

\end{table}

==> text/4.1.revisit.tex <==
\section{Revisiting Uni-Perceiver}
\label{sec:revisit}



%\subsection{Uni-Perceive for Generic Perception}
% Most previous  machine learning research  has focused on specific tasks or modalities, often with model architecture tailored to the task.
% However, it is difficult for task-specific paradigm  to accomplish collaboration across tasks and transfer to other tasks quickly, which  conflicts with designing a generic artificial perception model. 
% There are also some previous perception models  exploring  multi-modal representations learning and multi-task learning \cite{chen2020uniter,kim2021vilt}. But they still follow a task-specific paradigm, which focus on inputs from certain combination of modalities. 
% Moreover, they require task-specific heads specifically designed for each tasks, thus lacking the ability to zero-shot inference on novel tasks.

% To solve this problem,  Uni-Perceiver~\cite{zhu2021uniperceiver}, a generic perception architecture, is proposed to process a variety of modalities and tasks with unified modeling and shared parameters. 
% In Uni-Perceiver, the inputs and targets from arbitrary combinations of modalities are first converted into unified token sequence by lightweight modality-specific tokenizers such as the BPE tokenizer~\cite{sennrich2016neural} for text modality and the patch tokenizer~\cite{dosovitskiy2020image} for visual modality. Then the token sequnces are encoded into a unified representation space by a modality-agnostic  transformer encoder. 
%
% Uni-Perceiver also unify the task formulation for all perception tasks. Specifically, for a task with a set of inputs $\mathcal{X}$ and a set of candidate targets $\mathcal{Y}$, it is formulated to find the maximum likelihood target $y\in\mathcal{Y}$ for each input $x\in\mathcal{X}$ through the similarity of their representations:
To verify the effectiveness of the proposed XXX MoE, we apply it to Uni-Perceiver~\cite{zhu2021uniperceiver}, a generalist model that can process multiple modalities and tasks with shared parameters.

\noindent\textbf{Brief Review.~}
Overall, the key points of Uni-Perceiver are as follows:
%
(1) For multi-modality, inputs and targets from different modalities are converted into sequences of tokens and then encoded into a unified representation space by a modality-agnostic transformer encoder.
%
(2) 
% \jinguo{this part describes the unified task formulation for a single arbitrary task  $\{(\mathcal{X}, \mathcal{Y})\}$,  not multitask $\{(\mathcal{X}_i, \mathcal{Y}_i)\}_{i=1}^N$ }
% For multi-task,
To adapt to arbitrary tasks,
Uni-Perceiver reformulates tasks in different formats into a unified task formulation: given an input set $\mathcal{X}$ and candidate targets $\mathcal{Y}$, finding the maximum likelihood target $y\in\mathcal{Y}$ for each $x\in\mathcal{X}$ according to the similarity between their representations. Specifically, the unified task  can be summarized as Eqn. \eqref{eq:task}-\eqref{eq:jointp}.
\begin{equation}
\hat{y} = \arg\max_{y \in \mathcal{Y}} P(x, y),
\label{eq:task}
\end{equation}
\begin{equation}
P(x, y) \propto \exp\left(\cos\big(f(x), f(y)\big) / \tau \right),
\label{eq:jointp} 
\end{equation}
% where $f(\cdot)$ is the transformer encoder, and $\tau > 0$ is a learnable temperature parameter.
where $P(x, y)$ is the joint probability distribution calculated by the cosine similarity $\cos(\cdot)$ between the representation of $x$ and $y$, $f(\cdot)$ is the modality-agnostic transformer encoder, and $\tau$ is a learnable temperature parameter.
%
% \vspace{0.5em}\noindent\textbf{Pre-training on Multi-Modal Tasks.~}
% The unified formulation of Uni-Perceiver  eliminates the gap between the formulations of different perception tasks, which enables Uni-Perceiver to handle various modalities and tasks with a single shared model.
% To learn the generic representations from different modalities and tasks, Uni-Perceiver firstly constructs a large-scale pre-training dataset, which is a huge collections of various publicly-available datasets, including image-only datasets, video-only datasets, text-only datasets, and image-text-pair datasets.
%
% Then, Uni-Perceiver is pre-trained on a variety of multi-modality tasks simultaneously, including image/video classification, language modeling with/without image clues,  and image-text retrieval, \emph{etc}.
% All tasks for pre-training can be denoted as $\{\mathcal{X}_1, \mathcal{Y}_1\}, \{\mathcal{X}_2, \mathcal{Y}_2\}, ..., \{\mathcal{X}_n, \mathcal{Y}_n\}$, where $\mathcal{X}_i$ and $\mathcal{Y}_i$ is the input set and target set of the $i$-th task, respectively. 
(3) To share parameters among different modalites and tasks, Uni-Perceiver learns to model the joint distribution of inputs and targets from multi-modality tasks.
Here, we denote the pre-training tasks as $\{(\mathcal{X}_i, \mathcal{Y}_i)\}_{i=1}^N$, where $(\mathcal{X}_i, \mathcal{Y}_i)$ denotes the $i$-th task, $\mathcal{X}_i$ and $\mathcal{Y}_i$ represent the input and target set, respectively.  
The overall pre-training loss $L$ can be written as:
\begin{equation}
%\small
L = \sum_{i=1}^{N} \mathop{\mathbb{E}}_{(x, y) \in (\mathcal{X}_i, \mathcal{Y}_i)} \bigg(- \log \frac{P(x, y)}{\sum_{z \in \mathcal{Y}_i}{P(x, z)}}\bigg),
\end{equation}
where $\mathbb{E}$ is the mathematical expectation, and $(x, y)$ is an input-target pair sampled from the $i$-th task $(\mathcal{X}_i, \mathcal{Y}_i)$.
% Thanks to its generic formulations, Uni-Perceiver is able to train all tasks jointly, without introducing any other task-specific parameters and formulations, \emph{e.g.}, prediction heads.
%
% \vspace{0.5em}\noindent\textbf{Zero-shot, Prompt Tuning and Fine-Tuning.~}
% During the large-scale pre-training on multi-modality tasks, Uni-Perceiver learns to model the joint distribution of input and target from arbitrary modalites and tasks.
% Due to the generic perception modeling, Uni-Perceiver can perform zero-shot inference even on completely novel tasks that do not appear in the pre-training, \textit{i.e.,} video caption, video-text retrieval and visual-question-answering. 
% By converting those novel tasks into the unified task formulation,  Uni-Perceiver can obtain reasonable zero-shot performance.
% Furthermore, its performance can be boosted with additional task-specific data by prompt tuning~\cite{liuPtuningv2} and fine-tuning. 
% It can reach the performance close to SOTA results by prompt tuning with only a small amount of downstream data. It  can also be further improved to be on par with or superior to SOTA results by full-data finetuning.
(4) For downstream application, Uni-Perceiver can obtain reasonable zero-shot performance by converting new tasks into the base task format.
In addition, its performance can be boosted by few-data prompt tuning~\cite{liuPtuningv2} and full-data fine-tuning. 


% \vspace{0.5em}\noindent\textbf{Limitation: Modality and Task Interference.~}
\noindent\textbf{Limitation.~}
% Although Uni-Perceiver achieved promising performance on most tasks, it lags other task-specific SOTAs when transferred to a few novel tasks that do not appear in pre-training like GLUE, especially under zero-shot settings.
\jinguo{need to discuss}
Although Uni-Perceiver achieves promising performance on most tasks, \textcolor{red}{it lags behind other task-specific SOTAs when transferring to some new tasks that do not appear in pre-training, especially under zero-shot settings}.
%
% We speculate that Uni-Perceiver shares the parameters across different modalities and tasks, which may exacerbate task interference due to the capacity bottleneck~\cite{zhang2021share}.
We argue that this phenomenon is caused by the fully-shared parameters across modalities and tasks. Different modalities and tasks interfere with each other due to the limited model capacity~\cite{zhang2021share}.
% Increasing model capacity is known to be effective in multitask training \cite{kong2021multilingual}.
%
Increasing model capacity is an effective way to mitigate interference in multi-modality multi-task models~\cite{arivazhagan2019massively,kong2021multilingual}.
\textcolor{red}{As shown in Tab. {\color{red} x } and {\color{red} x }, when increasing the transformer encoder size from BERT\textsubscript{BASE} to BERT\textsubscript{LARGE}, the performance gain of Uni-Perceiver is more significant than those of other task-specific SOTAs.}
These results suggest that large model capacity is important for generalist models like Uni-Perceiver.
% can benefit more with increased model capacity.
However, directly increasing model capacity results in higher memory and computational costs, and the training and deploying of very large and dense networks is prohibitively expensive.
% Since every input example is processed by every parameter, 



% As shown in Tab.~\ref{tab:model_interference}, by switching the encoder from BERT\textsubscript{BASE} to BERT\textsubscript{LARGE}, Uni-Perceiver has a larger performance gain than task-specific SOTAs. These results indicating Uni-Perceiver can benefit more with increased model capacity.

% \input{tables/model_interference}



==> text/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Our code will be released once the paper is accepted, and the used data is publicly available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:exp}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Most experiments have stable results with little variance.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:exp}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the open datasets that we use.}
  \item Did you mention the license of the assets?
    \answerYes{See Section~\ref{sec:exp}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Our code will be released once the paper is accepted.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Section~\ref{sec:exp}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section~\ref{sec:exp}.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> text/method1.tex <==
% \section{Mixture-of-Experts for Uni-Perceiver}
\section{Methodology}
\label{sec:method}

\begin{figure}[t]
\centering
\includegraphics[width=0.98\textwidth]{figures/method.pdf}
\caption{Comparisons of fully-shared standard encoder block, task-specific encoder block with task-dedicated parameters, and encoder block with efficient MoE parameterization.}
\label{fig:differentencoderblock}
\vspace{-0.5em}
\end{figure}

% In this section, we aim to mitigate the issue of task interference in Uni-Perceiver. 
This work targets to mitigate the interference problem in
generalist models like Uni-Perceiver.
% Instead of directly increasing the size of shared model, which would significantly increase the memory and computational costs, we explore alternative unshared parameterization methods. These methods introduce some unshared parameters among different tasks to mitigate task interference with only negligible costs.
Instead of directly increasing the model size, which would drastically increase memory and computational cost, we explore Mixture of Experts (MoEs) for generalist models, and further propose Attribute-MoEs, which introduces parameters conditioned by  attributes of different levels to alleviate the interference issue with negligible overhead.



%introduce different candidate methods to mitigate task interference in Uni-Perceiver, without introducing prohibitively computation costs or harming the generality of Uni-Perceiver: Task-specific parameterization and Mixture of Experts with different routing strategies.
%We also discuss their trade-offs from the perspective of the training, inference, and transfer costs. 

\subsection{Generalist Model Architecture}
% Fig.~\ref{fig:differentencoderblock} illustrates the fully shared model used by the original Uni-Perceiver and other alternative unshared parameterization methods.
Fig.~\ref{fig:differentencoderblock} summarizes three mainstream architectures for general models: (1) standard architecture~\cite{zhu2021uniperceiver,jaegle2021perceiver,jaegle2021perceiver_} with parameters fully shared by different modalities and tasks, (2) task-specific 
% wwh: parameterization
parameterized
architecture~\cite{yuan2021florence,shao2021intern}\todo{more cites} equipped with dedicated parameters for each task to address the interference problem,
and (3) Mixture-of-Experts (MoE) architecture~\cite{shazeer2017outrageously,lepikhin2020gshard,fedus2021switch,kim2021scalable,vmoe}, which consists of a group of gated experts with separate parameters and mitigates the interference problem by dispatching different inputs to different experts.

%
% Fig.~\ref{fig:differentencoderblock}(a) shows the transformer encoder with fully shared parameters across different tasks, which suffers from task interference.
% Fig.~\ref{fig:differentencoderblock}(b) shows the na\"ive task-specific parameterization method, which preserves a set of dedicated parameters for each task. The separation of model parameters for different tasks can avoid task interference ideally. 
% Fig.~\ref{fig:differentencoderblock}(c) shows the more efficient Mixture-of-Experts (MoE) parameterization method, which consists of a group of experts with their separate parameters. MoE can mitigate task interference by dispatching different inputs to different experts.
% we will discuss these unshared parameterization methods as follows.

As discussed in Sec.~\ref{sec:revisit}, the standard architecture with fully shared parameters are widely used, but suffer from  modality and task interference problems.
Compared with the fully-shared architecture, the task-specific parameterized architecture mitigates the interference among different tasks, but hinders task-level collaboration and knowledge transfer, thus losing the advantages of multi-task training.
%
% wwh: 这里为啥ambiguous我没懂
% In addition, when transferring to down-stream tasks, task-specific parameterization is ambiguous to use which set of the taks-dedicated parameters. 
In addition, task-specific parameters hurt the generalization ability to novel tasks that did not appear in pre-training.
%, and the memory cost increase linearly with the number of involved tasks, which becomes inefficient and inconvenient as the number of tasks and the model size grow.
%
Unlike the above two architectures, the MoE architecture activates models sparsely according to different given inputs by selectively utilizing different subset of the model parameters.
% In addition to its contributions to the feasibility of training large models, MoE also provides a potential solution to mitigate task interference in shared models.
The sparse routing mechanism makes it possible to train very large generalist models, which maximizes the collaboration and meanwhile mitigates the interference problem.
% MoEs~\cite{shazeer2017outrageously,lepikhin2020gshard} has been successfully utilized in training large scale multi-lingual~\cite{fedus2021switch,kim2021scalable} and vision models~\cite{vmoe}.
In this work, we focus on exploring MoEs for general models and propose Attribute-MoEs whose experts are gated by different levels of attributes.




% \subsection{Task-Specific Parameterization}
% \label{sec:taskspecificparams}

% Task-specific parameterization is an effective way to reduce interference among different tasks, which has dedicated parameters for each task. As shown in Fig.~\ref{fig:differentencoderblock}(b), input tokens from the same task would be processed by a set of dedicated parameters, while inputs from different tasks would be dispatched to different modules. The separation of parameters results in an independent pathway for each task, thus avoid task interference ideally.
 
% Though the separation of parameters eliminates interference among different tasks, it also prevents the collaboration and knowledge transfer among tasks, thus losing the advantages of multi-tasking training. 
% When transferring to down-stream tasks, it is ambiguous to use which set of the taks-dedicated parameters. The task-specific parameterization also hinders the generalization ability to novel tasks that did not appear in pre-training.
% Moreover, task-specific parameters would increase linearly with the number of involved tasks, which becomes inefficient and inconvenient as the number of tasks and the model size grow.

\subsection{Conditional Mixture-of-Experts}

% The Mixture of Experts (MoE) \cite{shazeer2017outrageously,lepikhin2020gshard} architecture has been successfully utilized in training large scale multi-lingual \cite{fedus2021switch,kim2021scalable} and vision models \cite{vmoe}, which activates models sparsely according to different given inputs by selectively utilizing different subset of the model parameters.
% In addition to its contributions to the feasibility of training large models, MoE also provides a potential solution to mitigate task interference in shared models.
% The dynamic computation mechanism makes it possible to train a single large generic perception model, which maximizes the collaboration and meanwhile mitigates the interference among different tasks.
%; meanwhile, the  model with large-scale multitask and multi-modality pre-training can transfer to novel task with promising performance.

Without loss of generality, we explore the application of MoEs in the modality- and task-agnostic transformer of Uni-Perceiver.
% to mitigate the task interference.
% The transformer, which consists of alternating self-attention and dense feedforward network (FFN) layers, is the main part of the Uni-Perceiver and is used to  encode token sequnces from different task and different modality into a shared representation space.
Different from previous works~\cite{fedus2021switch,kim2021scalable,vmoe} that only add MoE layers to the FFN blocks, we replace linear projection layers in both self-attention and FFN blocks with MoE layers (see Fig.~\ref{fig:differentencoderblock}(c)), which is demonstrated to be crucial in mitigating the interference problem (\todo{ablations} See Appendix).

% MoE is implemented as \cite{vmoe}, which will be briefly introduced here.
Specifically, a prototype MoE layer is implemented as~\cite{vmoe}. Given any token $x_i$ in the input sequence $X=\{x_i\}_{i=1}^L$, with $E$ experts firstly introduces a gate decision vector $\mathcal{G} \in \mathbb{R}^E$ that dispatches different input tokens to different experts, which is calculated as:
\begin{equation}
\mathcal{G} = \operatorname{top}_k\left( \operatorname{softmax}\left(\mathbf{W}_g\cdot R(x_i)+ \epsilon \right)  \right).
\label{eq1}
\end{equation}
where $R(\cdot)$ defines the routing strategy for gate decision.
% , different $R(\cdot)$ indicates different routing strategy.
$\mathbf{W}_g$ is the trainable weights in gate decision and $\epsilon$ is the noise term. The $\operatorname{top}_k(\cdot)$ operator sets all values to be zero except the largest $k$ values.
Since $\mathcal{G}$  only has $k \ll E$ non-zero values, the token $x_i$ is routed to only a small number of experts. 
After getting the gate decision vector $\mathcal{G}$, the corresponding output $y_i$ is the weighted combinations of each expert's computation on $x_i$ as: %according to the gate decision $\mathcal{G}$ as
\begin{equation}
y_i =\sum_{e=1}^{E} \mathcal{G}_{e} \cdot \mathbf{W}_{e} \cdot x_i,
\label{eq2}
\end{equation}
where $\mathbf{W_e}$ is the linear projection weights of the $e$-th expert and  gate decision $\mathcal{G}_{e}$ determines how much the $e$-th expert contributes to the output $y_i$. Note that, experts with $\mathcal{G}_{e}=0$ does not need to be computed for saving computation.

%The MoE linear projection layer can be more computationally efficient since a new linear layer can parameterized as a weighed combination of all experts before applying the linear transformation, thus requiring computing only one expensive multiplication.
%By doing so, Eq. \ref{eq2} can be reformulated as 
%\begin{equation}
%\begin{aligned}
%    y_i &=\sum_{e=1}^{E} \left( \mathcal{G}_{e} \cdot \mathbf{W}_{e} \right) \cdot x_i \label{eq3}
%    \end{aligned}
%\end{equation}


% Besides to predict the weights of each expert in processing incoming token $x$,
% the  gate function $\operatorname{GATE(\cdot)}$  in MoE layer need satisfy two goals: (1) the balanced load of expert utilization  and (2) the efficiency at scale of gate function.
% The former goal is usually achieved by optimizing an auxiliary balancing loss, which is to encourage a balanced load across experts.
The routing strategy $R(\cdot)$ in Eqn.~\ref{eq1} plays an important role in the multi-modality and multi-task training of generalist models. By activating experts sparsely for different inputs, the MoE model can address the interference problem and keep the generality of the pre-training model.
In the remainder of this section, we would like to discuss plain routing strategies at different levels (see Fig. 2(a)-(d))
% (\emph{i.e.}, token-level, context-level, modality-level, and task-level) 
before introducing Attribute-MoE (see Fig. 2(e)).
% , which are also shown in Fig.~\ref{fig:routingstrategy}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.7\textwidth]{figures/bbb.jpg}
\caption{Comparisons of different routing strategies. We show an example of  the top-$1$ gate decisions under 2-task training.}
\label{fig:routingstrategy}
\vspace{-0.5em}
\end{figure}

\vspace{0.5em}\noindent\textbf{Token-Level Routing.~}
Following previous MoE Transformers~\cite{shazeer2017outrageously}, 
the token-Level MoE layer in our model directly use the token representation for the routing strategy, which can be written as:
\begin{equation}
    R_\text{token}(x_i) = x_i,
    \label{eq:r_token}
\end{equation}
% In Eqn.~\ref{eq:r_token}, we see that the gate decision for each token depends on the token representation itself.

\vspace{0.5em}\noindent\textbf{Context-Level Routing.~}
Since the similar tokens can appear in different sequences, there may be different optimal expert decisions even for the same token.
Therefore, we combine global context and local token representation to help gate function making more reliable decisions.
The routing strategy utilizing global context can be expressed as:
\begin{equation}
 R_\text{context}(x_i) =  \operatorname{concat}(x_i, \operatorname{attnpool}(X)),
\end{equation}
where $\operatorname{concat}(\cdot)$ indicates the concatenation operation,  $X=\{x_i\}_{i=1}^L$ is sequence of all tokens in the current sample, and $\operatorname{attnpool}(\cdot)$ indicates the attention pooling operator~\cite{clip}.
% the operator that first computes the global average pooling value of $X$, and then use a multi-head attention operation to compute global context, in which the query is the pooling feature and the keys are all the token representations of $X$.

\vspace{0.5em}\noindent\textbf{Modality-Level Routing.~}
Some works~\todo{cite} use modality-specific encoders with independent parameters for different modality inputs, and find that dedicated parameters for different modalities can boost task performance.
Inspire by this, we leverage the modality of current token as an alternative route strategy:
\begin{equation}
    R_\text{modal}(x_i) = \operatorname{embed}(\operatorname{id_\text{modal}}(x_i))
    \label{eq:r_modal}
\end{equation}
Here, $\operatorname{embed}(\cdot)$ represent the embedding layer, and $\operatorname{id}_\text{modal}(\cdot)$ indicates the modality index of current token $x_i$. In Eqn.~\ref{eq:r_modal}, the routing function will assign this token to experts according to its modality embedding.

\vspace{0.5em}\noindent\textbf{Task-Level Routing.~} 
Global task-level information can also be used to guide gate function making reliable decisions.
Following \cite{taskmoe}, the routing strategy can be formulated as follows:
\begin{equation}
    R_\text{task}(x_i) = \operatorname{embed}(\operatorname{id_{task}}(x_i)),
\end{equation}
where $\operatorname{id_{task}}(\cdot)$ is the task index of current token $x_i$. The task embedding for this task will be used to compute gate decision. 
Since  all tokens from one task have  the same task embedding, all tokens corresponding to this task will be routed to the same set of experts.

Among the aforementioned routing strategies, token-level, context-level and modality-level routing miss the information of current task, while task-level routing introduces task-specific id that hinders the generalization ability of Uni-Perceiver to down-steam tasks. To combine the advantages of different routing strategies, we propose to utilize token attributes to assist the gate decision.

\subsection{Attribute-MoE}
\input{tables/attributeid}

% \vspace{0.5em}\noindent\textbf{Attribute-MoE.~}
% Among the aforementioned routing strategies, token-level, context-level and modality-level routing miss the information of current task, while task-level routing introduces task-specific id that hinders the generalization ability of Uni-Perceiver to down-steam tasks. To combine the advantages of different routing strategies, we propose to utilize token attributes to assist the gate decision.
%
% Specifically, the attributes of the current token is represented as an 8-dimensional binary embedding, whose determined process is described in Tab.~\ref{tab:onehotforattribute}.
As described in Tab.~\ref{tab:onehotforattribute}, the attributes of the current token can be represented as an 8-dimensional binary embedding, whose attributes include the modalities of current task and token (see index 0-5), the forward type of the model (see index 6), and the token source (see index 7). To this end, the designed token attributes provide comprehensive information of current task meanwhile keep the task generalization ability. Based on the attribute embedding, the routing strategy of Attribute-MoE can be expressed as:
\begin{equation}
    R_\text{attr}(x_i) = \operatorname{layernorm} \left( \mathbf{W}_\text{attr} \cdot \operatorname{attr}(x_i) \right).
\end{equation}
Here, $\operatorname{attr}(x_i)$ is the 8-dimensional binary attribute embedding of the current token $x_i$ as described in Tab.~\ref{tab:onehotforattribute}. $\mathbf{W}_\text{attr} $ is the learnable weights to transform the attribute embedding to latent representation, and $\operatorname{layernorm}(\cdot)$ denotes a layer normalization~\cite{ba2016layer} for training stabilization.
% It obvious that the token attribute contains information from three granularities: task, modality, and token level.

% \subsection{Training, Inference, and Transfer Costs of Different Routing}

Fig.~\ref{fig:routingstrategy} shows different routing strategies. As shown in Fig.~\ref{fig:routingstrategy}(a)(b), token-level and context-level routing strategies are data-dependent, where each token can be routed to different experts independently.
On the other hand, as shown in Fig.~\ref{fig:routingstrategy}(c)(d)(e), modality-level, task-level, and attribute-level routing strategies are data-independent, where a set of tokens with the same ids would be routed to the same expert.
Among these data-independent routing strategies, only the task-level routing in Fig.~\ref{fig:routingstrategy}(d) has task-specific design, which leads to the same issue of poor generalization ability as the task-specific parameterization when transferring to down-steam tasks.

\xizhou{todo: modify follows}

\vspace{0.5em}\noindent\textbf{Token-level and Context-level Routing.~}
These two data-dependent routing strategies can increase the model capacity and flexibility since each token has its own independent pathway. But they also bring high memory cost  to model training. The entire model may be beyond the memory limit of a single accelerator device when the activated sub-network increases.  
 Model parallelism is usually needed to relieve memory cost by partitioning experts across multiple accelerators,  further introducing heavy inter-device  communication overhead.
What's more,  this problem persists when the pre-training model is employed to inference on trained tasks or transfer to other  tasks: all experts need to be loaded in memory and may be activated by any token.

\vspace{0.5em}\noindent\textbf{Task-level Routing.~}
By assigning different task embeddings to different  tasks, MoE model with task-level routing can be able to separate the parameters among different tasks  if interference exists.
Unlike task-specific parameterization in Sec.~\ref{sec:taskspecificparams}, it also permits the collaboration and knowledge transfer across tasks, for which different tasks can share the optimal experts.

Since only top-$k$ experts need to be activated for all tokens from current task, this data-independent routing strategy have excellent training and inference efficiency compared with data-dependent routing strategies.
% The efficiency of data-independent routing strategies can be further exploited by extracting out a sub-network to a particular task seen in the training stage.
% Only $k$ experts are preserved for computation in each MoE layer while other experts can be discarded for memory saving.
Moreover, since our experts all are  linear transformations, one new linear layer can be reparameterized before inference computation, whose weight is the weighted combination of all experts' weights by the gate value.
In this case, the computation cost of the network with  reparameterized MoE layers will be equivalent to a dense model without MoE but with higher task performance.
However, the task-specific design of task embedding prevents the task-level MoE model  from generalizing to other tasks smoothly, as the task embedding for this new task needs to be learned.


% \vspace{0.5em}\noindent\textbf{Data-Independent Routing.~}
% Data-Independent have excellent training and inference efficiency compared with data-dependent routings.
% The efficiency of data-independent routing strategies can be further exploited by extracting out a sub-network to a particular task seen in the training stage.
% Only $k$ experts are preserved for computation in each MoE layer while other experts can be discarded for memory saving.
% Moreover, since our experts all are  linear transformations, one new linear layer can be reparameterized before inference computation, whose weight is the weighted combination of all experts' weights by the gate value.
% In this case, the computation cost of the network with  reparameterized MoE layer will equivalent to dense model without MoE, but with higher task performance.

\vspace{0.5em}\noindent\textbf{Modality-level and attribute-level Routing.~}
These two routing strategies not only inherit the high efficiency   of task-level routing on training and inference but also can maintain the generalization ability as neither of them has a task-specific parameterization.
They both can transfer  to down-stream tasks and can conduct zero-shot inference on novel tasks that not appear during pre-training without any task-specific modification.

% \vspace{0.5em}\noindent\textbf{Transferring to Down-Stream Tasks.~}
% When transferring to other novel tasks that not be seen in the training,   MoE model with either token-level, context level, task-level, or modality-level routing,  lacks the ability to generalize to new tasks and need to be further tuned. 
% Besides, the prohibitive burden from memory and communication costs existing during training  remains in the transfer stage, for which the pre-training model still need to be loaded completely.
% The task-level routing MoE may be able to pick the best one sub-network for the new task from the existing task embedding, but this is a suboptimal choise due to the task gap.
% However, because our attribute embedding encodes the task, modality, and token information simultaneously,  the transfer  efficiency of  attribute MoE can  be guaranteed by extracting out a sub-network    depending on the attribute embedding  for the new task. Then zero-shot inference or further tuning  of the new task can be conducted smoothly.
%  Therefore, it is efficient to transfer the attribute-level routing MoE to novel tasks, especially in zero-shot and few-shot scenarios.
 
 

